Neural Importance Sampling

We propose to use deep neural networks for generating samples in Monte Carlo integration. Our work is based on non-linear independent components estimation (NICE), which we extend in numerous ways to improve performance and enable its application to integration problems. First, we introduce piecewise-polynomial coupling transforms that greatly increase the modeling power of individual coupling layers. Second, we propose to preprocess the inputs of neural networks using one-blob encoding, which stimulates localization of computation and improves inference. Third, we derive a gradient-descent-based optimization for the KL and the $\chi^2$ divergence for the specific application of Monte Carlo integration with unnormalized stochastic estimates of the target distribution. Our approach enables fast and accurate inference and efficient sample generation independently of the dimensionality of the integration domain. We show its benefits on generating natural images and in two applications to light-transport simulation: first, we demonstrate learning of joint path-sampling densities in the primary sample space and importance sampling of multi-dimensional path prefixes thereof. Second, we use our technique to extract conditional directional densities driven by the product of incident illumination and the BSDF in the rendering equation, and we leverage the densities for path guiding. In all applications, our approach yields on-par or higher performance than competing techniques at equal sample count.

==> fig-path-guiding-thesis-1.tex <==
\setlength{\fboxrule}{10pt}%
\setlength{\insetvsep}{20pt}%
\setlength{\tabcolsep}{-1pt}%
\renewcommand{\arraystretch}{1}%
\small%
\hspace*{-2mm}%
\begin{tabular}{ccccccccc}
  & & & & & \multicolumn{2}{c}{Ours, KL divergence} & Ours, $\chi^2$ div. \\
  \cmidrule(lr){6-7}
  & & PT-Unidir & PPG & GMM & NPG-Radiance & NPG-Product & NPG-Product & Reference \\
    \setInset{A}{red}{55}{140}{51}{38}%
    \setInset{B}{orange}{440}{120}{51}{38}%
    \rotatebox{90}{\hspace{-1.75cm}\Bathroom{}}\hspace{0.14cm} & 
    \addBeautyCrop{images/references-thesis-1/glossy-bathroom-Reference.jpg}{0.27}{640}{360}{0}{0}{640}{360} &
    \addInsets{images/fig-path-guiding-thesis-1/glossy-bathroom-PT-unidir.jpg} &
    \addInsets{images/fig-path-guiding-thesis-1/glossy-bathroom-PPG.jpg} &
    \addInsets{images/fig-path-guiding-thesis-1/glossy-bathroom-Vorba.jpg} &
    \addInsets{images/fig-path-guiding-thesis-1/glossy-bathroom-Ours-IRS.jpg} &
    \addInsets{images/fig-path-guiding-thesis-1/glossy-bathroom-Ours-FPS.jpg} &
    \addInsets{images/fig-path-guiding-thesis-1/glossy-bathroom-Ours-FPS-chi.jpg} &
    \addInsets{images/references-thesis-1/glossy-bathroom-Reference.jpg} \\
  & \multicolumn{1}{r}{MAPE:} & 0.1467 & 0.1893 & 0.2718 & 0.1780 & \textbf{0.0542} & 0.0655 \\[2pt]
    \setInset{A}{red}{260}{10}{51}{38}%
    \setInset{B}{orange}{540}{320}{51}{38}%
    \rotatebox{90}{\hspace{-1.75cm}\Bedroom{}}\hspace{0.14cm} & 
    \addBeautyCrop{images/references-thesis-1/bedroom-Reference.jpg}{0.27}{640}{360}{0}{0}{640}{360} &
    \addInsets{images/fig-path-guiding-thesis-1/bedroom-PT-unidir.jpg} &
    \addInsets{images/fig-path-guiding-thesis-1/bedroom-PPG.jpg} &
    \addInsets{images/fig-path-guiding-thesis-1/bedroom-Vorba.jpg} &
    \addInsets{images/fig-path-guiding-thesis-1/bedroom-Ours-IRS.jpg} &
    \addInsets{images/fig-path-guiding-thesis-1/bedroom-Ours-FPS.jpg} &
    \addInsets{images/fig-path-guiding-thesis-1/bedroom-Ours-FPS-chi.jpg} &
    \addInsets{images/references-thesis-1/bedroom-Reference.jpg} \\
  & \multicolumn{1}{r}{MAPE:} & 0.0778 & 0.0530 & 0.0628 & 0.0449 & \textbf{0.0317} & 0.0421 \\[2pt]
    \setInset{A}{red}{55}{220}{51}{38}%
    \setInset{B}{orange}{430}{90}{51}{38}%
    \rotatebox{90}{\hspace{-1.75cm}\Bookshelf{}}\hspace{0.14cm} & 
    \addBeautyCrop{images/references-thesis-1/bookshelf-Reference.jpg}{0.27}{640}{360}{0}{0}{640}{360} &
    \addInsets{images/fig-path-guiding-thesis-1/bookshelf-PT-unidir.jpg} &
    \addInsets{images/fig-path-guiding-thesis-1/bookshelf-PPG.jpg} &
    \addInsets{images/fig-path-guiding-thesis-1/bookshelf-Vorba.jpg} &
    \addInsets{images/fig-path-guiding-thesis-1/bookshelf-Ours-IRS.jpg} &
    \addInsets{images/fig-path-guiding-thesis-1/bookshelf-Ours-FPS.jpg} &
    \addInsets{images/fig-path-guiding-thesis-1/bookshelf-Ours-FPS-chi.jpg} &
    \addInsets{images/references-thesis-1/bookshelf-Reference.jpg} \\
  & \multicolumn{1}{r}{MAPE:} & 0.7955 & 0.1251 & \textbf{0.0982} & 0.1136 & 0.1196 & 0.1682 \\[2pt]
    \setInset{A}{red}{450}{110}{51}{38}%
    \setInset{B}{orange}{160}{245}{51}{38}%
    \rotatebox{90}{\hspace{-2.20cm}\CopperHairball{}}\hspace{0.14cm} & 
    \addBeautyCrop{images/references-thesis-1/hairball-Reference.jpg}{0.27}{640}{360}{0}{0}{640}{360} &
    \addInsets{images/fig-path-guiding-thesis-1/hairball-PT-unidir.jpg} &
    \addInsets{images/fig-path-guiding-thesis-1/hairball-PPG.jpg} &
    \addInsets{images/fig-path-guiding-thesis-1/hairball-Vorba.jpg} &
    \addInsets{images/fig-path-guiding-thesis-1/hairball-Ours-IRS.jpg} &
    \addInsets{images/fig-path-guiding-thesis-1/hairball-Ours-FPS.jpg} &
    \addInsets{images/fig-path-guiding-thesis-1/hairball-Ours-FPS-chi.jpg} &
    \addInsets{images/references-thesis-1/hairball-Reference.jpg} \\
  & \multicolumn{1}{r}{MAPE:} & 0.4685 & 0.1275 & 0.1561 & 0.1420 & \textbf{0.0855} & 0.1379 \\[2pt]
    \setInset{A}{red}{296}{80}{51}{38}%
    \setInset{B}{orange}{406}{305}{51}{38}%
    \rotatebox{90}{\hspace{-2.00cm}\CornellBox{}}\hspace{0.14cm} & 
    \addBeautyCrop{images/references-thesis-1/cbox-Reference.jpg}{0.27}{868}{488}{0}{0}{868}{488} &
    \addInsets{images/fig-path-guiding-thesis-1/cbox-PT-unidir.jpg} &
    \addInsets{images/fig-path-guiding-thesis-1/cbox-PPG.jpg} &
    \addInsets{images/fig-path-guiding-thesis-1/cbox-Vorba.jpg} &
    \addInsets{images/fig-path-guiding-thesis-1/cbox-Ours-IRS.jpg} &
    \addInsets{images/fig-path-guiding-thesis-1/cbox-Ours-FPS.jpg} &
    \addInsets{images/fig-path-guiding-thesis-1/cbox-Ours-FPS-chi.jpg} &
    \addInsets{images/references-thesis-1/cbox-Reference.jpg} \\
  & \multicolumn{1}{r}{MAPE:} & 0.1845 & 0.0443 & 0.0490 & 0.0347 & \textbf{0.0212} & 0.0271 \\[2pt]
    \setInset{A}{red}{540}{230}{51}{38}%
    \setInset{B}{orange}{430}{320}{51}{38}%
    \rotatebox{90}{\hspace{-2.20cm}\CountryKitchen{}}\hspace{0.14cm} & 
    \addBeautyCrop{images/references-thesis-1/kitchen-Reference.jpg}{0.27}{640}{360}{0}{0}{640}{360} &
    \addInsets{images/fig-path-guiding-thesis-1/kitchen-PT-unidir.jpg} &
    \addInsets{images/fig-path-guiding-thesis-1/kitchen-PPG.jpg} &
    \addInsets{images/fig-path-guiding-thesis-1/kitchen-Vorba.jpg} &
    \addInsets{images/fig-path-guiding-thesis-1/kitchen-Ours-IRS.jpg} &
    \addInsets{images/fig-path-guiding-thesis-1/kitchen-Ours-FPS.jpg} &
    \addInsets{images/fig-path-guiding-thesis-1/kitchen-Ours-FPS-chi.jpg} &
    \addInsets{images/references-thesis-1/kitchen-Reference.jpg} \\
  & \multicolumn{1}{r}{MAPE:} & 0.6879 & 0.1299 & 0.1505 & 0.1204 & \textbf{0.0953} & 0.2411 \\[-5pt]
\end{tabular}
\unsetInset{A}%%
\unsetInset{B}%%

==> fig-path-guiding-thesis-2.tex <==
\setlength{\fboxrule}{10pt}%
\setlength{\insetvsep}{20pt}%
\setlength{\tabcolsep}{-1pt}%
\renewcommand{\arraystretch}{1}%
\small%
\hspace*{-2mm}%
\begin{tabular}{ccccccccc}
  & & & & & \multicolumn{2}{c}{Ours, KL divergence} & Ours, $\chi^2$ div. \\
  \cmidrule(lr){6-7}
  & & PT-Unidir & PPG & GMM & NPG-Radiance & NPG-Product & NPG-Product & Reference \\
    \setInset{A}{red}{280}{110}{51}{38}%
    \setInset{B}{orange}{480}{150}{51}{38}%
    \rotatebox{90}{\hspace{-1.65cm}\Necklace{}}\hspace{0.14cm} & 
    \addBeautyCrop{images/references-thesis-2/necklace-Reference.jpg}{0.27}{640}{360}{0}{0}{640}{360} &
    \addInsets{images/fig-path-guiding-thesis-2/necklace-PT-unidir.jpg} &
    \addInsets{images/fig-path-guiding-thesis-2/necklace-PPG.jpg} &
    \addInsets{images/fig-path-guiding-thesis-2/necklace-Vorba.jpg} &
    \addInsets{images/fig-path-guiding-thesis-2/necklace-Ours-IRS.jpg} &
    \addInsets{images/fig-path-guiding-thesis-2/necklace-Ours-FPS.jpg} &
    \addInsets{images/fig-path-guiding-thesis-2/necklace-Ours-FPS-chi.jpg} &
    \addInsets{images/references-thesis-2/necklace-Reference.jpg} \\
  & \multicolumn{1}{r}{MAPE:} & 0.3436 & 0.1632 & 0.1612 & 0.1629 & \textbf{0.1273} & 0.3104 \\[2pt]
    \setInset{A}{red}{150}{220}{51}{38}%
    \setInset{B}{orange}{440}{320}{51}{38}%
    \rotatebox{90}{\hspace{-2.20cm}\SalleDeBain{}}\hspace{0.14cm} & 
    \addBeautyCrop{images/references-thesis-2/bathroom2-Reference.jpg}{0.27}{640}{360}{0}{0}{640}{360} &
    \addInsets{images/fig-path-guiding-thesis-2/bathroom2-PT-unidir.jpg} &
    \addInsets{images/fig-path-guiding-thesis-2/bathroom2-PPG.jpg} &
    \addInsets{images/fig-path-guiding-thesis-2/bathroom2-Vorba.jpg} &
    \addInsets{images/fig-path-guiding-thesis-2/bathroom2-Ours-IRS.jpg} &
    \addInsets{images/fig-path-guiding-thesis-2/bathroom2-Ours-FPS.jpg} &
    \addInsets{images/fig-path-guiding-thesis-2/bathroom2-Ours-FPS-chi.jpg} &
    \addInsets{images/references-thesis-2/bathroom2-Reference.jpg} \\
  & \multicolumn{1}{r}{MAPE:} & 0.1846 & 0.0713 & 0.0798 & 0.0572 & \textbf{0.0421} & 0.0621 \\[2pt]
    \setInset{A}{red}{185}{76}{51}{38}%
    \setInset{B}{orange}{140}{230}{51}{38}%
    \rotatebox{90}{\hspace{-1.70cm}\Spaceship{}}\hspace{0.14cm} & 
    \addBeautyCrop{images/references-thesis-2/spaceship-Reference.jpg}{0.27}{540}{304}{0}{0}{540}{304} &
    \addInsets{images/fig-path-guiding-thesis-2/spaceship-PT-unidir.jpg} &
    \addInsets{images/fig-path-guiding-thesis-2/spaceship-PPG.jpg} &
    \addInsets{images/fig-path-guiding-thesis-2/spaceship-Vorba.jpg} &
    \addInsets{images/fig-path-guiding-thesis-2/spaceship-Ours-IRS.jpg} &
    \addInsets{images/fig-path-guiding-thesis-2/spaceship-Ours-FPS.jpg} &
    \addInsets{images/fig-path-guiding-thesis-2/spaceship-Ours-FPS-chi.jpg} &
    \addInsets{images/references-thesis-2/spaceship-Reference.jpg} \\
  & \multicolumn{1}{r}{MAPE:} & 0.0422 & 0.0346 & 0.0640 & 0.0340 & \textbf{0.0202} & 0.0490 \\[2pt]
    \setInset{A}{red}{450}{110}{51}{38}%
    \setInset{B}{orange}{300}{195}{51}{38}%
    \rotatebox{90}{\hspace{-2.20cm}\Sponza{}}\hspace{0.14cm} & 
    \addBeautyCrop{images/references-thesis-2/sponza-Reference.jpg}{0.27}{640}{360}{0}{0}{640}{360} &
    \addInsets{images/fig-path-guiding-thesis-2/sponza-PT-unidir.jpg} &
    \addInsets{images/fig-path-guiding-thesis-2/sponza-PPG.jpg} &
    \addInsets{images/fig-path-guiding-thesis-2/sponza-Vorba.jpg} &
    \addInsets{images/fig-path-guiding-thesis-2/sponza-Ours-IRS.jpg} &
    \addInsets{images/fig-path-guiding-thesis-2/sponza-Ours-FPS.jpg} &
    \addInsets{images/fig-path-guiding-thesis-2/sponza-Ours-FPS-chi.jpg} &
    \addInsets{images/references-thesis-2/sponza-Reference.jpg} \\
  & \multicolumn{1}{r}{MAPE:} & 1.7086 & 0.3528 & 0.1151 & \textbf{0.1094} & 0.1103 & 0.2474 \\[2pt]
    \setInset{A}{red}{470}{40}{51}{38}%
    \setInset{B}{orange}{360}{235}{51}{38}%
    \rotatebox{90}{\hspace{-2.05cm}\SwimmingPool{}}\hspace{0.14cm} & 
    \addBeautyCrop{images/references-thesis-2/pool-Reference.jpg}{0.27}{640}{360}{0}{0}{640}{360} &
    \addInsets{images/fig-path-guiding-thesis-2/pool-PT-unidir.jpg} &
    \addInsets{images/fig-path-guiding-thesis-2/pool-PPG.jpg} &
    \addInsets{images/fig-path-guiding-thesis-2/pool-Vorba.jpg} &
    \addInsets{images/fig-path-guiding-thesis-2/pool-Ours-IRS.jpg} &
    \addInsets{images/fig-path-guiding-thesis-2/pool-Ours-FPS.jpg} &
    \addInsets{images/fig-path-guiding-thesis-2/pool-Ours-FPS-chi.jpg} &
    \addInsets{images/references-thesis-2/pool-Reference.jpg} \\
  & \multicolumn{1}{r}{MAPE:} & 0.6878 & 0.0824 & 0.0772 & 0.0770 & \textbf{0.0655} & 0.0870 \\[2pt]
    \setInset{A}{red}{296}{80}{51}{38}%
    \setInset{B}{orange}{426}{305}{51}{38}%
    \rotatebox{90}{\hspace{-2.30cm}\GlossyCornellBox{}}\hspace{0.14cm} & 
    \addBeautyCrop{images/references-thesis-2/glossy-cbox-Reference.jpg}{0.27}{868}{488}{0}{0}{868}{488} &
    \addInsets{images/fig-path-guiding-thesis-2/glossy-cbox-PT-unidir.jpg} &
    \addInsets{images/fig-path-guiding-thesis-2/glossy-cbox-PPG.jpg} &
    \addInsets{images/fig-path-guiding-thesis-2/glossy-cbox-Vorba.jpg} &
    \addInsets{images/fig-path-guiding-thesis-2/glossy-cbox-Ours-IRS.jpg} &
    \addInsets{images/fig-path-guiding-thesis-2/glossy-cbox-Ours-FPS.jpg} &
    \addInsets{images/fig-path-guiding-thesis-2/glossy-cbox-Ours-FPS-chi.jpg} &
    \addInsets{images/references-thesis-2/glossy-cbox-Reference.jpg} \\
  & \multicolumn{1}{r}{MAPE:} & 1.2277 & 0.1411 & 0.0793 & \textbf{0.0591} & 0.0648 & 0.1097 \\[-5pt]
\end{tabular}
\unsetInset{A}%%
\unsetInset{B}%%

==> fig-pss-guiding-thesis-1.tex <==
\setlength{\fboxrule}{10pt}%
\setlength{\insetvsep}{20pt}%
\setlength{\tabcolsep}{-1pt}%
\renewcommand{\arraystretch}{1}%
\small%
\hspace*{-2mm}%
\begin{tabular}{ccccccccc}
  & & & & Affine, $\nlayers=16$ & \multicolumn{3}{c}{Ours, piecewise-quadratic, $\nlayers=4$} \\
  \cmidrule(lr){6-8}
  & & PT-Unidir & PSSPS---4D & NPS---6D & NPS---2D & NPS---4D & NPS---6D & Reference \\
    \setInset{A}{red}{55}{140}{51}{38}%
    \setInset{B}{orange}{440}{120}{51}{38}%
    \rotatebox{90}{\hspace{-1.75cm}\Bathroom{}}\hspace{0.14cm} & 
    \addBeautyCrop{images/fig-pss-guiding-thesis-1/glossy-bathroom-Reference.jpg}{0.27}{640}{360}{0}{0}{640}{360} &
    \addInsets{images/fig-pss-guiding-thesis-1/glossy-bathroom-PT-unidir.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-1/glossy-bathroom-PSSPS.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-1/glossy-bathroom-Affine-4d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-1/glossy-bathroom-Ours-2d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-1/glossy-bathroom-Ours-4d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-1/glossy-bathroom-Ours-6d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-1/glossy-bathroom-Reference.jpg} \\
  & \multicolumn{1}{r}{MAPE:} & 0.1467 & \textbf{0.1426} & 0.1529 & 0.1474 & 0.1450 & 0.1460 \\[2pt]
    \setInset{A}{red}{260}{10}{51}{38}%
    \setInset{B}{orange}{540}{320}{51}{38}%
    \rotatebox{90}{\hspace{-1.75cm}\Bedroom{}}\hspace{0.14cm} & 
    \addBeautyCrop{images/fig-pss-guiding-thesis-1/bedroom-Reference.jpg}{0.27}{640}{360}{0}{0}{640}{360} &
    \addInsets{images/fig-pss-guiding-thesis-1/bedroom-PT-unidir.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-1/bedroom-PSSPS.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-1/bedroom-Affine-4d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-1/bedroom-Ours-2d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-1/bedroom-Ours-4d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-1/bedroom-Ours-6d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-1/bedroom-Reference.jpg} \\
  & \multicolumn{1}{r}{MAPE:} & 0.0778 & 0.0678 & 0.0778 & 0.0711 & \textbf{0.0678} & 0.0684 \\[2pt]
    \setInset{A}{red}{55}{220}{51}{38}%
    \setInset{B}{orange}{430}{90}{51}{38}%
    \rotatebox{90}{\hspace{-1.75cm}\Bookshelf{}}\hspace{0.14cm} & 
    \addBeautyCrop{images/fig-pss-guiding-thesis-1/bookshelf-Reference.jpg}{0.27}{640}{360}{0}{0}{640}{360} &
    \addInsets{images/fig-pss-guiding-thesis-1/bookshelf-PT-unidir.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-1/bookshelf-PSSPS.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-1/bookshelf-Affine-4d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-1/bookshelf-Ours-2d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-1/bookshelf-Ours-4d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-1/bookshelf-Ours-6d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-1/bookshelf-Reference.jpg} \\
  & \multicolumn{1}{r}{MAPE:} & 0.7955 & 0.7553 & 0.6712 & 0.6915 & \textbf{0.6702} & 0.6810 \\[2pt]
    \setInset{A}{red}{450}{110}{51}{38}%
    \setInset{B}{orange}{160}{245}{51}{38}%
    \rotatebox{90}{\hspace{-2.20cm}\CopperHairball{}}\hspace{0.14cm} & 
    \addBeautyCrop{images/fig-pss-guiding-thesis-1/hairball-Reference.jpg}{0.27}{640}{360}{0}{0}{640}{360} &
    \addInsets{images/fig-pss-guiding-thesis-1/hairball-PT-unidir.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-1/hairball-PSSPS.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-1/hairball-Affine-4d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-1/hairball-Ours-2d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-1/hairball-Ours-4d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-1/hairball-Ours-6d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-1/hairball-Reference.jpg} \\
  & \multicolumn{1}{r}{MAPE:} & 0.4685 & 0.3139 & 0.2400 & 0.2236 & 0.1987 & \textbf{0.1956} \\[2pt]
    \setInset{A}{red}{296}{80}{51}{38}%
    \setInset{B}{orange}{406}{305}{51}{38}%
    \rotatebox{90}{\hspace{-2.00cm}\CornellBox{}}\hspace{0.14cm} & 
    \addBeautyCrop{images/fig-pss-guiding-thesis-1/cbox-Reference.jpg}{0.27}{868}{488}{0}{0}{868}{488} &
    \addInsets{images/fig-pss-guiding-thesis-1/cbox-PT-unidir.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-1/cbox-PSSPS.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-1/cbox-Affine-4d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-1/cbox-Ours-2d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-1/cbox-Ours-4d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-1/cbox-Ours-6d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-1/cbox-Reference.jpg} \\
  & \multicolumn{1}{r}{MAPE:} & 0.1845 & 0.1305 & 0.1419 & 0.1299 & \textbf{0.1086} & 0.1093 \\[2pt]
    \setInset{A}{red}{540}{230}{51}{38}%
    \setInset{B}{orange}{430}{320}{51}{38}%
    \rotatebox{90}{\hspace{-2.20cm}\CountryKitchen{}}\hspace{0.14cm} & 
    \addBeautyCrop{images/fig-pss-guiding-thesis-1/kitchen-Reference.jpg}{0.27}{640}{360}{0}{0}{640}{360} &
    \addInsets{images/fig-pss-guiding-thesis-1/kitchen-PT-unidir.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-1/kitchen-PSSPS.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-1/kitchen-Affine-4d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-1/kitchen-Ours-2d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-1/kitchen-Ours-4d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-1/kitchen-Ours-6d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-1/kitchen-Reference.jpg} \\
  & \multicolumn{1}{r}{MAPE:} & 0.6879 & 0.6476 & 0.6607 & 0.6598 & 0.6033 & \textbf{0.5633} \\[-5pt]
\end{tabular}
\unsetInset{A}%%
\unsetInset{B}%%

==> fig-pss-guiding-thesis-2.tex <==
\setlength{\fboxrule}{10pt}%
\setlength{\insetvsep}{20pt}%
\setlength{\tabcolsep}{-1pt}%
\renewcommand{\arraystretch}{1}%
\small%
\hspace*{-2mm}%
\begin{tabular}{ccccccccc}
  & & & & Affine, $\nlayers=16$ & \multicolumn{3}{c}{Ours, piecewise-quadratic, $\nlayers=4$} \\
  \cmidrule(lr){6-8}
  & & PT-Unidir & PSSPS---4D & NPS---6D & NPS---2D & NPS---4D & NPS---6D & Reference \\
    \setInset{A}{red}{280}{110}{51}{38}%
    \setInset{B}{orange}{480}{150}{51}{38}%
    \rotatebox{90}{\hspace{-1.65cm}\Necklace{}}\hspace{0.14cm} & 
    \addBeautyCrop{images/fig-pss-guiding-thesis-2/necklace-Reference.jpg}{0.27}{640}{360}{0}{0}{640}{360} &
    \addInsets{images/fig-pss-guiding-thesis-2/necklace-PT-unidir.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-2/necklace-PSSPS.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-2/necklace-Affine-4d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-2/necklace-Ours-2d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-2/necklace-Ours-4d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-2/necklace-Ours-6d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-2/necklace-Reference.jpg} \\
  & \multicolumn{1}{r}{MAPE:} & 0.3436 & 0.3334 & 0.3349 & \textbf{0.2210} & 0.2594 & 0.2680 \\[2pt]
    \setInset{A}{red}{150}{220}{51}{38}%
    \setInset{B}{orange}{440}{320}{51}{38}%
    \rotatebox{90}{\hspace{-2.20cm}\SalleDeBain{}}\hspace{0.14cm} & 
    \addBeautyCrop{images/fig-pss-guiding-thesis-2/bathroom2-Reference.jpg}{0.27}{640}{360}{0}{0}{640}{360} &
    \addInsets{images/fig-pss-guiding-thesis-2/bathroom2-PT-unidir.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-2/bathroom2-PSSPS.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-2/bathroom2-Affine-4d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-2/bathroom2-Ours-2d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-2/bathroom2-Ours-4d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-2/bathroom2-Ours-6d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-2/bathroom2-Reference.jpg} \\
  & \multicolumn{1}{r}{MAPE:} & 0.1846 & 0.1606 & 0.1833 & 0.1703 & 0.1591 & \textbf{0.1581} \\[2pt]
    \setInset{A}{red}{185}{76}{51}{38}%
    \setInset{B}{orange}{140}{230}{51}{38}%
    \rotatebox{90}{\hspace{-1.70cm}\Spaceship{}}\hspace{0.14cm} & 
    \addBeautyCrop{images/fig-pss-guiding-thesis-2/spaceship-Reference.jpg}{0.27}{540}{304}{0}{0}{540}{304} &
    \addInsets{images/fig-pss-guiding-thesis-2/spaceship-PT-unidir.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-2/spaceship-PSSPS.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-2/spaceship-Affine-4d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-2/spaceship-Ours-2d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-2/spaceship-Ours-4d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-2/spaceship-Ours-6d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-2/spaceship-Reference.jpg} \\
  & \multicolumn{1}{r}{MAPE:} & 0.0422 & 0.0331 & 0.0343 & \textbf{0.0259} & 0.0259 & 0.0261 \\[2pt]
    \setInset{A}{red}{450}{110}{51}{38}%
    \setInset{B}{orange}{300}{195}{51}{38}%
    \rotatebox{90}{\hspace{-2.20cm}\Sponza{}}\hspace{0.14cm} & 
    \addBeautyCrop{images/fig-pss-guiding-thesis-2/sponza-Reference.jpg}{0.27}{640}{360}{0}{0}{640}{360} &
    \addInsets{images/fig-pss-guiding-thesis-2/sponza-PT-unidir.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-2/sponza-PSSPS.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-2/sponza-Affine-4d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-2/sponza-Ours-2d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-2/sponza-Ours-4d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-2/sponza-Ours-6d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-2/sponza-Reference.jpg} \\
  & \multicolumn{1}{r}{MAPE:} & 1.7086 & 1.6916 & 1.6353 & \textbf{1.3217} & 1.4673 & 1.6161 \\[2pt]
    \setInset{A}{red}{470}{40}{51}{38}%
    \setInset{B}{orange}{360}{235}{51}{38}%
    \rotatebox{90}{\hspace{-2.05cm}\SwimmingPool{}}\hspace{0.14cm} & 
    \addBeautyCrop{images/fig-pss-guiding-thesis-2/pool-Reference.jpg}{0.27}{640}{360}{0}{0}{640}{360} &
    \addInsets{images/fig-pss-guiding-thesis-2/pool-PT-unidir.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-2/pool-PSSPS.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-2/pool-Affine-4d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-2/pool-Ours-2d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-2/pool-Ours-4d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-2/pool-Ours-6d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-2/pool-Reference.jpg} \\
  & \multicolumn{1}{r}{MAPE:} & 0.6878 & 0.4941 & 0.3863 & 0.2052 & \textbf{0.1872} & 0.1976 \\[2pt]
    \setInset{A}{red}{296}{80}{51}{38}%
    \setInset{B}{orange}{426}{305}{51}{38}%
    \rotatebox{90}{\hspace{-2.30cm}\GlossyCornellBox{}}\hspace{0.14cm} & 
    \addBeautyCrop{images/fig-pss-guiding-thesis-2/glossy-cbox-Reference.jpg}{0.27}{868}{488}{0}{0}{868}{488} &
    \addInsets{images/fig-pss-guiding-thesis-2/glossy-cbox-PT-unidir.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-2/glossy-cbox-PSSPS.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-2/glossy-cbox-Affine-4d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-2/glossy-cbox-Ours-2d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-2/glossy-cbox-Ours-4d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-2/glossy-cbox-Ours-6d.jpg} &
    \addInsets{images/fig-pss-guiding-thesis-2/glossy-cbox-Reference.jpg} \\
  & \multicolumn{1}{r}{MAPE:} & 1.2277 & 1.2001 & 1.3622 & 0.8037 & \textbf{0.7964} & 1.1081 \\[-5pt]
\end{tabular}
\unsetInset{A}%%
\unsetInset{B}%%
